LABELMAKER: Automatic Semantic Label Generation from RGB-D Trajectories

Semantic annotations are indispensable to train or evaluate perception models, yet very costly to acquire. This work introduces a fully automated 2D/3D labeling framework that, without any human intervention, can generate labels for RGB-D scans at equal (or better) level of accuracy than comparable manually annotated datasets such as ScanNet. Our approach is based on an ensemble of state-of-the-art segmentation models and 3D lifting through neural rendering. We demonstrate the effectiveness of our LabelMaker pipeline by generating significantly better labels for the ScanNet datasets and automatically labelling the previously unlabeled ARKitScenes dataset. Code and models are available at https://labelmaker.org

==> sections/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tables/ablation_2d_models.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{r|ccc}
    \toprule
                    &  mIoU & mAcc & tAcc \\
        \midrule
        w/o OVSeg \cite{ovseg} & 0.371 & 0.447 & 0.718 \\
        w/o Mask3D \cite{mask3d} & 0.288 & 0.365 & 0.656 \\
        w/o InternImage \cite{} & 0.370 & 0.455 & 0.690 \\
        w/o CMX \cite{} & 0.380 & 0.444 & 0.719 \\
        w/o ScanNet \cite{scannet} & 0.291 & 0.357 & 0.635 \\
        Consensus (ours) & 0.389 & 0.483 & 0.770 \\
        \name (ours) & 0.391 & 0.493 & 0.772 \\
    \bottomrule
    \end{tabular}  
    \caption{Leave one out of the 2D model, eval only on the 3D, eval on our scannet labels} 
    \label{tab:ablation_2d_models}
\end{table}
